Relative induction principles for type theories

We present new induction principles for the syntax of dependent type theories, which we call relative induction principles. The result of the induction principle relative to a functor F into the syntax is stable over the codomain of F. We rely on the internal language of presheaf categories. In order to combine the internal languages of multiple presheaf categories, we use Dependent Right Adjoints and Multimodal Type Theory. Categorical gluing is used to prove these induction principles, but it not visible in their statements, which involve a notion of model without context extensions. As example applications of these induction principles, we give short and boilerplate-free proofs of canonicity and normalization for some small type theories, and sketch proofs of other metatheoretic results.

==> macros.tex <==
%%% General macros

% Abbreviations.
\makeatletter
\newcommand{\DeclareAbbrevation}[2]{\newcommand{#1}{\@ifnextchar{.}{#2}{#2.\@\xspace}}}
\makeatother

\DeclareAbbrevation{\ie}{i.e}
\DeclareAbbrevation{\eg}{e.g}
\DeclareAbbrevation{\cf}{cf}
\DeclareAbbrevation{\etc}{etc}
\DeclareAbbrevation{\resp}{resp}
\DeclareAbbrevation{\etal}{et al}
\DeclareAbbrevation{\ibid}{ibid}
\DeclareAbbrevation{\ca}{ca}
\DeclareAbbrevation{\vs}{vs}

% Lowercase mathcal
\DeclareFontFamily{U}{mathc}{}
\DeclareFontShape{U}{mathc}{m}{it}%
{<->s*[1.03] mathc10}{}
\DeclareMathAlphabet{\mathcal}{U}{mathc}{m}{it}

% Japanese letters (for the Yoneda embedding)
\DeclareFontFamily{U}{min}{}
\DeclareFontShape{U}{min}{m}{n}{<-> udmj30}{}

% Emphasis
\newcommand{\defemph}[1]{\textbf{#1}}

% Double langle/rangle
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
  \mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
  \mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother

% Arrows
\newcommand{\uda}{\updownarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\hra}{\hookrightarrow}
\newcommand{\rat}{\rightarrowtail}
\newcommand{\ratri}{\rightarrowtriangle}
\newcommand{\thra}{\twoheadrightarrow}
\newcommand{\thla}{\twoheadleftarrow}
\newcommand{\rsqa}{\rightsquigarrow}

% Brackets
\newcommand{\abs}[1]{{\left| #1 \right|}}
\newcommand{\sem}[1]{{\llbracket #1 \rrbracket}}
\newcommand{\lens}[1]{{\llparenthesis #1 \rrparenthesis}}
\newcommand{\trunc}[1]{{\parallel #1 \parallel}}
\newcommand{\angles}[1]{{\left\langle #1 \right\rangle}}
\newcommand{\uquote}[1]{{\ulcorner #1 \urcorner}}
\newcommand{\dquote}[1]{{\dlcorner #1 \drcorner}}

%%% TIKZ macros

% used for 2-cells
\tikzset{shorten <>/.style={shorten >=#1,shorten <=#1}}

%%% Category theory

% Categorical operations
\newcommand{\Ob}{\mathsf{Ob}}
\newcommand{\Hom}{\mathsf{Hom}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\op}{\mathsf{op}}

% Yoneda embedding & Psh categories
\newcommand{\yo}{\text{\usefont{U}{min}{m}{n}\symbol{'210}}}
\newcommand{\psh}[1]{\ensuremath{\widehat{#1}}}

% Short names for models (mathbb)
\newcommand{\MA}{\mathbb{A}}
\newcommand{\MB}{\mathbb{B}}
\newcommand{\MC}{\mathbb{C}}
\newcommand{\MD}{\mathbb{D}}
\newcommand{\ME}{\mathbb{E}}
\newcommand{\MF}{\mathbb{F}}
\newcommand{\MG}{\mathbb{G}}
\newcommand{\MH}{\mathbb{H}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MJ}{\mathbb{J}}
\newcommand{\MK}{\mathbb{K}}
\newcommand{\ML}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\MN}{\mathbb{N}}
\newcommand{\MO}{\mathbb{O}}
\newcommand{\MP}{\mathbb{P}}
\newcommand{\MQ}{\mathbb{Q}}
\newcommand{\MR}{\mathbb{R}}
\newcommand{\MS}{\mathbb{S}}
\newcommand{\MT}{\mathbb{T}}
\newcommand{\MU}{\mathbb{U}}
\newcommand{\MV}{\mathbb{V}}
\newcommand{\MW}{\mathbb{W}}
\newcommand{\MX}{\mathbb{X}}
\newcommand{\MY}{\mathbb{Y}}
\newcommand{\MZ}{\mathbb{Z}}

% Short names for sets and internal things (mathrm / mathsf)
\newcommand{\SProp}{\mathrm{Prop}}
\newcommand{\SSet}{\mathrm{Set}}
\newcommand{\SCat}{\mathrm{Cat}}
\newcommand{\SPsh}{\mathrm{Psh}}
\newcommand{\SRepPsh}{\mathrm{RepPsh}}

\newcommand{\SA}{\mathsf{A}}
\newcommand{\SB}{\mathsf{B}}
\newcommand{\SC}{\mathsf{C}}
\newcommand{\SD}{\mathsf{D}}
\newcommand{\SE}{\mathsf{E}}
\newcommand{\SF}{\mathsf{F}}
\newcommand{\SG}{\mathsf{G}}
\newcommand{\SH}{\mathsf{H}}
\newcommand{\SI}{\mathsf{I}}
\newcommand{\SJ}{\mathsf{J}}
\newcommand{\SK}{\mathsf{K}}
\newcommand{\SL}{\mathsf{L}}
\newcommand{\SM}{\mathsf{M}}
\newcommand{\SN}{\mathsf{N}}
\newcommand{\SO}{\mathsf{O}}
\newcommand{\SP}{\mathsf{P}}
\newcommand{\SQ}{\mathsf{Q}}
\newcommand{\SR}{\mathsf{R}}
\renewcommand{\SS}{\mathsf{S}}
\newcommand{\ST}{\mathsf{T}}
\newcommand{\SU}{\mathsf{U}}
\newcommand{\SV}{\mathsf{V}}
\newcommand{\SW}{\mathsf{W}}
\newcommand{\SX}{\mathsf{X}}
\newcommand{\SY}{\mathsf{Y}}
\newcommand{\SZ}{\mathsf{Z}}

% Short names for categories (mathbf or mathcal)
\newcommand{\CSet}{\mathbf{Set}}
\newcommand{\CProp}{\mathbf{Prop}}
\newcommand{\CPsh}{\mathbf{Psh}}
\newcommand{\CDepPsh}{\mathbf{DepPsh}}
\newcommand{\CCat}{\mathbf{Cat}}
\newcommand{\CCwf}{\mathbf{CwF}}
\newcommand{\CMod}{\mathbf{Mod}}

\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CE}{\mathcal{E}}
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CI}{\mathcal{I}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CM}{\mathcal{M}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CO}{\mathcal{O}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CQ}{\mathcal{Q}}
\newcommand{\CR}{\mathcal{R}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CW}{\mathcal{W}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\CZ}{\mathcal{Z}}

\newcommand{\BA}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\BC}{\mathbf{C}}
\newcommand{\BD}{\mathbf{D}}
\newcommand{\BE}{\mathbf{E}}
\newcommand{\BF}{\mathbf{F}}
\newcommand{\BG}{\mathbf{G}}
\newcommand{\BH}{\mathbf{H}}
\newcommand{\BI}{\mathbf{I}}
\newcommand{\BJ}{\mathbf{J}}
\newcommand{\BK}{\mathbf{K}}
\newcommand{\BL}{\mathbf{L}}
\newcommand{\BM}{\mathbf{M}}
\newcommand{\BN}{\mathbf{N}}
\newcommand{\BO}{\mathbf{O}}
\newcommand{\BP}{\mathbf{P}}
\newcommand{\BQ}{\mathbf{Q}}
\newcommand{\BR}{\mathbf{R}}
\newcommand{\BS}{\mathbf{S}}
\newcommand{\BT}{\mathbf{T}}
\newcommand{\BU}{\mathbf{U}}
\newcommand{\BV}{\mathbf{V}}
\newcommand{\BW}{\mathbf{W}}
\newcommand{\BX}{\mathbf{X}}
\newcommand{\BY}{\mathbf{Y}}
\newcommand{\BZ}{\mathbf{Z}}

%
\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}

%%% Type theory

% Components of models of type theory
\newcommand{\type}{\mathsf{type}}
\newcommand{\Con}{\mathsf{Con}}
\newcommand{\Sub}{\mathsf{Sub}}
\newcommand{\Ty}{\mathsf{Ty}}
\newcommand{\ty}{\mathsf{ty}}
\newcommand{\Tm}{\mathsf{Tm}}
\newcommand{\tm}{\mathsf{tm}}
\newcommand{\Var}{\mathsf{Var}}
\newcommand{\var}{\mathsf{var}}

% Booleans
\newcommand{\Bool}{\mathbb{B}}
\newcommand{\BoolTy}{\mathbf{B}}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\elimBool}{\mathsf{elim}_{\BoolTy}}

% Natural numbers
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\NatTy}{\mathbf{N}}
\newcommand{\zero}{\mathsf{zero}}
\newcommand{\suc}{\mathsf{suc}}
\newcommand{\elimNat}{\mathsf{elim}_{\NatTy}}

% Id-types
\newcommand{\Id}{\mathsf{Id}}
\newcommand{\J}{\mathsf{J}}
\newcommand{\refl}{\mathsf{refl}}

% Eq-types
\newcommand{\Eq}{\mathsf{Eq}}

% Equivalences / hLevels
\newcommand{\Equiv}{\mathrm{Equiv}}
\newcommand{\isEquiv}{\mathrm{isEquiv}}
\newcommand{\isContr}{\mathrm{isContr}}
\newcommand{\isProp}{\mathrm{isProp}}
\newcommand{\isSet}{\mathrm{isSet}}
\newcommand{\isLinv}{\mathrm{isLInv}}
\newcommand{\isRinv}{\mathrm{isRInv}}

% Pi-types
\newcommand{\app}{\mathsf{app}}
\newcommand{\lam}{\mathsf{lam}}
\newcommand{\funext}{\mathsf{funext}}

% Sigma and Unit-types
\newcommand{\pair}{\mathsf{pair}}
\newcommand{\fst}{\mathsf{fst}}
\newcommand{\snd}{\mathsf{snd}}

\newcommand{\Unit}{\mathbf{1}}
\renewcommand{\tt}{\mathsf{tt}}

\newcommand{\Init}{\mathbf{0}}
\newcommand{\absurd}{\mathsf{absurd}}

% Quotients
\newcommand{\Quot}{\mathbf{Q}}
\newcommand{\quot}{\mathbf{q}}

% Universes
\newcommand{\UU}{\mathcal{U}}
\newcommand{\UV}{\mathcal{V}}
\newcommand{\El}{\mathsf{El}}
\newcommand{\Lift}{\mathsf{Lift}}
\newcommand{\lift}{\mathsf{lift}}


%%% Macros specific to this document

% Misc
\newcommand{\inv}{^{-1}}
\newcommand{\Th}{\MT}
\newcommand{\isRep}{\mathrm{isRep}}

% Circled dollar symbol
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.1pt] (char) {#1};}}
\newcommand{\circleddollar}{\mathbin{\circled{\scalebox{0.7}{$\$$}}}}

% Normalization
\newcommand{\CRen}{\mathcal{Ren}}
\newcommand{\NfTy}{\mathsf{NfTy}}
\newcommand{\nfty}{\mathsf{nfty}}
\newcommand{\Ne}{\mathsf{Ne}}
\renewcommand{\ne}{\mathsf{ne}}
\newcommand{\Nf}{\mathsf{Nf}}
\newcommand{\nf}{\mathsf{nf}}
\newcommand{\norm}{\mathsf{norm}}
\newcommand{\stab}{\mathsf{stab}}
\newcommand{\HasNTy}{\mathsf{HasNTy}}
\newcommand{\HasNe}{\mathsf{HasNe}}
\newcommand{\HasNf}{\mathsf{HasNf}}

% Colors
\newcommand{\modcolor}[1]{\textcolor{orange!60!black}{#1}}
\newcommand{\natcolor}[1]{\textcolor{teal}{#1}}
\newcommand{\tickcolor}[1]{\textcolor{white!70!black}{#1}}

% MTT
% \newcommand{\lock}[2]{\mbox{\faLock}^{\tickcolor{#1}}_{\modcolor{#2}}}
% \newcommand{\unlock}[2]{\mbox{\faUnlock}^{\tickcolor{#1}}_{\modcolor{#2}}}
% \newcommand{\key}[3]{{\mbox{\faKey}\natcolor{#1} : \tickcolor{#2} \Ra \tickcolor{#3}}}
% \newcommand{\keyeq}[3]{{\mbox{\faKey}\natcolor{#1} : \tickcolor{#2} = \tickcolor{#3}}}
% \newcommand{\keyiso}[3]{{\mbox{\faKey}\natcolor{#1} : \tickcolor{#2} \simeq \tickcolor{#3}}}

\newcommand{\mmod}[1]{\{\modcolor{#1}\}}
\newcommand{\smod}[1]{\{\tickcolor{#1}\}}
\newcommand{\emod}[2]{\{\tickcolor{#1} \colon\modcolor{#2}\}}

\newcommand{\mkey}[1]{[\natcolor{#1}]}
\newcommand{\skey}[2]{[\tickcolor{#1} / \tickcolor{#2}]}
\newcommand{\smkey}[2]{[\modcolor{#1} / \modcolor{#2}]}
\newcommand{\ekey}[3]{[\natcolor{#1} \colon\tickcolor{#2} / \tickcolor{#3}]}
\newcommand{\emkey}[3]{[\natcolor{#1} \colon\modcolor{#2} / \modcolor{#3}]}

% Ambrus
\newcommand{\K}{\mathsf{K}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

